Entropy-regularized Diffusion Policy with Q-Ensembles for Offline Reinforcement Learning

This paper presents advanced techniques of training diffusion policies for offline reinforcement learning (RL). At the core is a mean-reverting stochastic differential equation (SDE) that transfers a complex action distribution into a standard Gaussian and then samples actions conditioned on the environment state with a corresponding reverse-time SDE, like a typical diffusion policy. We show that such an SDE has a solution that we can use to calculate the log probability of the policy, yielding an entropy regularizer that improves the exploration of offline datasets. To mitigate the impact of inaccurate value functions from out-of-distribution data points, we further propose to learn the lower confidence bound of Q-ensembles for more robust policy improvement. By combining the entropy-regularized diffusion policy with Q-ensembles in offline RL, our method achieves state-of-the-art performance on most tasks in D4RL benchmarks. Code is available at https://github.com/ruoqizzz/Entropy-Regularized-Diffusion-Policy-with-QEnsemble.

==> sections/method_sde.tex <==


\section{Training and Sampling with Mean-reverting SDE}
\label{sec:tsde}
Below we explain the training process and the sampling process of a diffusion policy with the meaning-reverting SDE. 
We start with the forward process, explaining the diffusion loss which is the behavior cloning loss in our case. Then, we introduce how to generate actions from the learned policy. 

\subsection{Training Process of Diffusion Policy}



Similar to other score-based models~\citep{song2020score,ho2020denoising}, the generative process of our SDE starts from a standard Gaussian noise and then simulates the corresponding reverse-time SDE following \eqref{eq:reverse-sde} as
\begin{equation}
    \diff {a} = \big[ -\theta_t \, a - \sigma_t^2 \, \nabla_x \log p_t(a) \big] \diff t + \sigma_t \diff \bar{w}.
    \label{eq:reverse-irsde}
\end{equation}
\blue{(Maybe we can remove it to the Appendix since we didn't use it.)}

During training, the initial diffusion state $a(0)$ is given ($a\sim \mathcal{D}\cond s$ in our case) and thus we can obtain the ground truth score $\nabla_{a}\log p_t(a)$ based on the marginal distribution \eqref{eq:margin_p}:
\begin{equation}
    \nabla_{{a}}\log p_t({a} \cond {a}(0)) = - \frac{{a}(t) - {a}(0) \expp^{-\bar{\theta}_{t}}}{1 - \expp^{-2 \, \bar{\theta}_{t}}},
    \label{eq:score}
\end{equation}
which can be approximated using a neural network and optimized with score-matching loss. Moreover, the marginal distribution \eqref{eq:margin_p} gives the reparameterization of the state:
\begin{equation}
    a(t) = a(0)\expp^{-\bar{\theta}_{t}} + \sqrt{1 - \expp^{-2\bar{\theta}_{t}}} \cdot \bm{\epsilon}_t,
    \label{eq:reparameterize_xt}
\end{equation}
where $\bm{\epsilon}_t$ is a standard Gaussian noise $\bm{\epsilon}_t \sim \mathcal{N}(0, \mathbf{I})$. By substituting \eqref{eq:reparameterize_xt} into \eqref{eq:score}, the score function can be re-written in terms of the noise as
\begin{equation}
    \nabla_{{a}}\log p_t({a} \cond {a}(0)) = - \frac{\bm{\epsilon}_t}{\sqrt{1 - \expp^{-2 \, \bar{\theta}_{t}}}}.
    \label{eq:noise-score}
\end{equation}
Then we follow the practical settings in diffusion models~\citep{ho2020denoising,dhariwal2021diffusion} to estimate the noise with a time-dependent neural network $\tilde{\bm{\epsilon}}_\phi(s)$ and optimize it with a simplified noise matching loss:
\begin{equation}
    L(\phi) \coloneqq \mathbb{E}_{\tau \in [0, T]} \Big[ \big\lVert \tilde{\bm{\epsilon}}^{(\tau)}_\phi(a_0\expp^{-\bar{\theta}_{\tau}} + \sqrt{1 - \expp^{-2\bar{\theta}_{\tau}}} \cdot \bm{\epsilon}_i) - \bm{\epsilon}_i) \bigr\rVert\Big],
    \label{eq:noise_objective}
\end{equation}
where $\tau$ is a randomly sampled timestep and $\{{a}^\tau\}_{\tau=0}^T$ denotes the discretization of the diffusion process. 


==> tab/alpha-other.tex <==
\small
\begin{wraptable}{r}{0.55\textwidth}
\centering
\scriptsize
\caption{Ablation experiments of our method on \textbf{Gym},  \textbf{Adroit}, and \textbf{Kitchen} tasks with different entropy temperatures. }
\label{table:alpha-other}
% \small
\begin{tabular}{l|cccccc}
\toprule
 Entropy temperature $\alpha$ & 0  & 0.01 & 0.05 & 0.1 & auto \\
% \midrule
% Antmaze-umaze-diverse-v0& 78.3 & 79.8& \textbf{84.0} & 79.3 & 81.8\\
% Antmaze-medium-play-v0 & 85.7 & \textbf{91.4}& 91 & 88.3 & 92.0\\
% Antmaze-medium-diverse-v0& 89.0 & 91.6 & 90.7 &\textbf{93.5} & 90.8 \\
% Antmaze-large-play-v0  & 77.7 & 81.2 & 78.3& \textbf{82} & 82.0\\
% Antmaze-large-diverse-v0 & 73.7 & 76.4 & 71.3 & \textbf{78.3} & 76.0 \\
% \bottomrule
\midrule
HalfCheetah-Medium-v2  & 53.7 &54.9  &54.0   &\textbf{55.3} & 54.2 \\
Hopper-Medium-v2     & 94.8 &94.2   &93.3   &\textbf{97.7 } &  94.0 \\
Walker2D-Medium-v2    & 89.6   &\textbf{92.5}  &91.6   &89.9& 91.9\\
\midrule
pen-human-v1    & 60.9  & 67.2 &63.6& 69.8& \textbf{77.8} \\
pen-cloned-v1      & 57.9  & 66.3 & 61.8& 56.5&  \textbf{77.8}\\
\midrule
Kitchen-complete-v0      &80.6   &82.3 & 77.6&54.4 & \textbf{84.4} \\
Kitchen-Mixed-v0      & 57.0   & \textbf{60.2} & 50.8 & 56.5 &  \\
\bottomrule
\end{tabular}
\end{wraptable}
\normalsize

==> tab/alpha.tex <==
\small
\begin{table}[t]
\centering
\tiny
\caption{Ablation experiments of our method on \textbf{Gym},  \textbf{Antmaze-}, \textbf{Adroit}, and \textbf{Kitchen} tasks with different entropy temperatures. }
\label{table:alpha-other}
\small
\begin{tabular}{l|cccccc}
\toprule
 Entropy temperature $\alpha$ & 0  & 0.01 & 0.05 & 0.1 & auto \\
\midrule
Antmaze-umaze-diverse-v0& 78.3 & 79.8& \textbf{84.0} & 79.3 & 81.8\\
Antmaze-medium-play-v0 & 85.7 & \textbf{91.4}& 91 & 88.3 & 92.0\\
Antmaze-medium-diverse-v0& 89.0 & 91.6 & 90.7 &\textbf{93.5} & 90.8 \\
Antmaze-large-play-v0  & 77.7 & 81.2 & 78.3& \textbf{82} & 82.0\\
Antmaze-large-diverse-v0 & 73.7 & 76.4 & 71.3 & \textbf{78.3} & 76.0 \\
% \bottomrule
\midrule
HalfCheetah-Medium-v2  & 53.7 &54.9  &54.0   &\textbf{55.3} & 54.2 \\
Hopper-Medium-v2     & 94.8 &94.2   &93.3   &\textbf{97.7 } &  94.0 \\
Walker2D-Medium-v2    & 89.6   &\textbf{92.5}  &91.6   &89.9& 91.9\\
\midrule
pen-human-v1    & 60.9  & 67.2 &63.6& 69.8& \textbf{77.8} \\
pen-cloned-v1      & 57.9  & 66.3 & 61.8& 56.5&  \textbf{77.8}\\
\midrule
Kitchen-complete-v0      &80.6   &82.3 & 77.6&54.4 & \textbf{84.4} \\
Kitchen-Mixed-v0      & 57.0   & \textbf{60.2} & 50.8 & 56.5 &  \\
\bottomrule
\end{tabular}
\end{table}
\normalsize

==> tab/overall_res.tex <==
\begin{table}[t]
    \centering

% \begin{table}[t]
\begin{minipage}{1.\linewidth}
% \vspace{-1em}
\centering
\scriptsize
\caption{Average normalized scores on D4RL benchmark tasks. Results of BC, CQL, IQL, and IQL+EDP are taken directly from \citet{kang2023edp}, and all other results are taken from their original papers. Our results are reported by averaging 5 random seeds.}
\label{table:overall_res}
\centering
\vspace{0.5em}
% \begin{center}
% \begin{small}
% \begin{sc}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{l|ccccccc|c}
\toprule
Gym Tasks & BC  & DT  & CQL  & IQL  & IDQL-A  & IQL+EDP   & Diff-QL&   Ours \\
\midrule
Halfcheetah-medium-v2 & 42.6 & 42.6 & 44.0   & 47.4  & 51.0    & 48.1 & 51.1 &   \textbf{54.9} \\
Hopper-medium-v2  & 52.9 & 67.6 & 58.5 & 66.3 & 65.4    & 63.1 & 90.5    &\textbf{94.2} \\
Walker2d-medium-v2    & 75.3 & 74.0 & 72.5 & 78.3 & 82.5    & 85.4 & 87.0  &    \textbf{92.5}\\
Halfcheetah-medium-replay-v2& 36.6 & 36.6 & 45.5 & 44.2 & 45.9    & 43.8 & 47.8   &\textbf{57.0} \\
Hopper-medium-replay-v2 & 18.1 & 82.7 & 95.0   & 94.7 & 92.1    & 99.1 & 101.3 &  \textbf{102.7} \\
Walker2d-medium-replay-v2   & 26.0 & 66.6   & 77.2 & 73.9 & 85.1    & 84.0   & \textbf{95.5}   & 94.2 \\
Halfcheetah-medium-expert-v2& 55.2 & 86.8 & 91.6 & 86.7 & 95.9    & 86.7 & \textbf{96.8}   & 90.3 \\
Hopper-medium-expert-v2 & 52.5 & 107.6 & 105.4  & 91.5 & 108.6    & 99.6 & 111.1 &  \textbf{111.9} \\
Walker2d-medium-expert-v2   & 107.5 & 108.1  & 108.8  & 109.6  & \textbf{112.7}   & 109.0 & 110.1  & 111.2 \\
\midrule
\textbf{Average} & 51.9 & 74.7 & 77.6& 77.0&   82.1   & 79.9& 88.0  & \textbf{89.9} \\
\bottomrule
\toprule
Adroit Tasks & BC  & BCQ  & BEAR & CQL  & IQL   & IQL+EDP   & Diff-QL&   Ours\\
\midrule
% Adroit  \\
Pen-human-v1   & 63.9 & 68.9 & -1.0 & 37.5 & 71.5  & 72.7 & \textbf{72.8 }  & 67.2 \\
Pen-cloned-v1  & 37.0 & 44.0 & 26.5 & 39.2 & 37.3  & \textbf{70.0 }  & 57.3   & 66.3 \\
\midrule
\textbf{Average} & 50.5 & 56.5 & 12.8 & 38.4 & 54.4  & \textbf{71.4}  & 65.1  & 66.8\\
\bottomrule
\toprule
Kitchen Tasks & BC  & BCQ  & BEAR & CQL  & IQL   & IQL+EDP   & Diff-QL&   Ours\\
\midrule
% Kitchen \\
kitchen-complete-v0   & 65.0 & 8.1 & 0.0 & 43.8 & 62.5  & 75.5 & \textbf{84}   & 82.3 \\
kitchen-partial-v0    & 38.0 & 18.9 & 13.1 & 49.8 & 46.3  & 46.3 & \textbf{60.5}  & 60.3 \\
kitchen-mixed-v0  & 51.5 & 8.1 & 47.2 & 51   & 51  & 56.5 & \textbf{62.6} &  60.2 \\
\midrule
\textbf{Average} & 51.5 & 11.7 & 20.1 & 48.2 & 53.3  & 59.4& \textbf{69.0} &  68.5  \\
\bottomrule

\end{tabular}
}
% \end{sc}
% \end{small}
\end{minipage}

\begin{minipage}{1.\linewidth}
% \begin{table}[t]
\centering
\scriptsize
\caption{Average normalized scores on D4RL \textbf{AntMaze} tasks. Results of BC, DT, CQL, IQL, and IQL+EDP are taken directly from \citet{kang2023edp}, and all other results are taken from their original papers. Our results are reported by averaging 5 random seeds.}
\label{table:antmaze_res}
\vspace{0.5em}
% \begin{center}
% \begin{small}
% \begin{sc}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{l|cccccccc|c}
\toprule
AntMaze Tasks & BC  & DT  & CQL  & IQL  & MSG & IDQL-A & IQL+EDP   & Diff-QL&  Ours\\
\midrule
Antmaze-umaze-v0  & 54.6 & 59.2 & 74   & 87.5 & 97.8 & 94.0 & 87.5 & 93.4  &  \textbf{100}\\
Antmaze-umaze-diverse-v0    & 45.6 & 53.0 & 84.0   & 62.2 &\textbf{ 81.8} & 80.2 & 62.2 & 66.2  & 79.8 \\
Antmaze-medium-play-v0  & 0.0  & 0.0  & 61.2 & 71.2 & 89.6 & 84.5 & 71.2 & 76.6  &  \textbf{91.4}\\
Antmaze-medium-diverse-v0   & 0.0 & 0.0    & 53.7 & 70.0   & 88.6 & 84.8 & 70.0   & 78.6  & \textbf{91.6} \\
Antmaze-large-play-v0 & 0.0  & 0.0  & 15.8 & 39.6 & 72.6 & 63.5 & 39.6 & 46.4  & \textbf{81.2} \\
Antmaze-large-diverse-v0    & 0.0 & 0.0    & 14.9 & 47.5 & 71.4 & 67.9 & 47.6 & 56.6  &  \textbf{76.4}\\
\midrule
\textbf{Average} & 16.7 & 18.7 & 50.6 & 63.0   & 83.6 & 79.1 & 63.0& 69.6 &  \textbf{86.7}\\
\bottomrule

\end{tabular}
}
% \end{sc}
% \end{small}
% \end{center}
\vspace{-1em}
\end{minipage}
\end{table}

==> tab/q-en_stability_plot.tex <==
\begin{figure}
    \centering
    \begin{minipage}{0.55\textwidth}
        \centering
% \scriptsize
\caption{Comparison of our entropy-based diffusion policy with different ensemble sizes on select AntMaze tasks.}
\label{table:q-ensemble}
% \begin{center}
% \begin{small}
% \begin{sc}
\begin{tabular}{lccc}
\toprule
   Ensemble Size      & $1$   & $4$    &  $64$ \\
\midrule
antmaze-medium-play-v0      & $50.2$  & $87.2$     &$\textbf{91.4}$\\
antmaze-medium-diverse-v0   & $67.2$   & $87.2$     &$\textbf{91.6}$\\
antmaze-large-play-v0       & $48.2$  & $52.4$ &$\textbf{81.2}$\\ 
antmaze-large-diverse-v0      & $58.8$  & $69.0$ &
$\textbf{76.4}$\\
\midrule
\textbf{Average}            & 56.1  & 74.0     &\textbf{85.2}\\
\bottomrule
\end{tabular}
    \end{minipage}
    % figure
    \begin{minipage}{0.4\textwidth}
    \centering
    % \footnotesize
    \includegraphics[width=1.\linewidth]{figs/ql-eql-2x2.pdf}
    \caption{Comparison of learning curves between Diffusion-QL and our method on Antmaze tasks over 5 random seeds. Our method shows better empirical stability across four tasks. }
    \label{fig:ql-eql}
    \end{minipage}
\end{figure}
